SelectLLM: Can LLMs Select Important Instructions to Annotate?

Instruction tuning benefits from large and diverse datasets; however, creating such datasets involves a high cost of human labeling. While synthetic datasets generated by large language models (LLMs) have partly solved this issue, they often contain low-quality data. One effective solution is selectively annotating unlabelled instructions, especially given the relative ease of acquiring unlabeled instructions or texts from various sources. However, how to select unlabelled instructions is not well-explored, especially in the context of LLMs. Therefore, we introduce SelectLLM, an alternative framework that leverages the capabilities of LLMs to select unlabeled instructions more effectively. Specifically, SelectLLM consists of two key steps: Coreset-based clustering of unlabelled instructions for enlarging diversity and prompting of LLM to identify the most beneficial instructions within each cluster. We evaluate SelectLLM on AlpacaEval2 and MT-Bench, demonstrating its ability to outperform state-of-the-art methods like Alpagasus. In addition, we compare the performance and compatibility of SelectLLM with various LLMs, such as ChatGPT, LLaMA-3.1-70B, and Gemma-2-27b. SelectLLM's adaptability and robustness are further evidenced by its ability to maintain high performance across both human and synthetic datasets. All code and data are publicly available (https://github.com/minnesotanlp/select-llm).

==> 3_preliminary.tex <==
\section{Preliminary}

\subsection{Task description}

We first describe the problem setup of our interest.
Let $\mathcal{X}=\{x_{i}\}_{i=1}^{M}$ denote the given un-annotated dataset, where $x_{i}$ represents $i$th instruction example.  
Then, our goal is to select $N$ most effective instructions from $\mathcal{X}$ which will be labeled by human annotators, to fine-tune a given large language model (LLM) $f_{\theta}$, \textit{e.g.}, LLaMA-2 \citep{touvron2023llama}, and make it be generalized for various instructions.
Specifically, let's assume that we select $N$ instructions under a criteria $s(j)$:  
\begin{align}
    &\mathcal{X}(S)=\{x_{s(j)}\}_{j=1}^{N}, \nonumber \\
    &~\text{where}~S=\{s(j)|s(j) \in [1,M]\}_{j=1}^{N}
\end{align}
where $S$ is the indices of selected instructions.
Then, the selected instruction $x \in \mathcal{X}(S)$ is labeled with a corresponding response $y$ by human annotators, and it results in the annotated instruction dataset $\mathcal{D}$, where $\mathcal{D}=\{(x_{s(j)},y_{s(j)})\}_{j=1}^{N}$.
\footnote{
We assume that the human responses could be obtained right after the selection for the experiments.} 
Therefore, the performance of fine-tuned LLMs on $\mathcal{X}(S)$ is significantly varied depending on which selection criteria $s(j)$ is considered. 
While various criterion has been explored under tasks like active learning (see Section \ref{sec:2}), this direction is less explored under the regime of instruction tuning.

\subsection{Selection by prompting LLMs}




==> figures/Figure3_embeddings.tex <==
\begin{figure*}[t]
\begin{center}
    {
    \subfigure[Random]
        {
        \includegraphics[width=0.31\textwidth]{figures/raw_files/temp.png}
        \label{fig:embed_rand}
        }
    \subfigure[Baseline]
        {
        \includegraphics[width=0.31\textwidth]{figures/raw_files/temp.png}
        \label{fig:embed_base}
        }
    \subfigure[Ours]
        {
        \includegraphics[width=0.31\textwidth]{figures/raw_files/temp.png}
        \label{fig:embed_ours}
        } \quad
    \subfigure[Ours]
        {
        \includegraphics[width=0.31\textwidth]{figures/raw_files/temp.png}
        \label{fig:embed_ours}
        }
    }
\end{center}
\caption{Embedding.
}
\label{fig:embed_results}
\end{figure*}

==> figures/Figure4_examples.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=1.1\textwidth,clip]{figures/raw_files/Examples.pdf}
    \caption{Inferences from \textit{SelectLLM}, Random, and Coreset methods for the given instruction. \textit{SelectLLM} is able to do a better reasoning, as highlighted by the green text. Red text shows proper salutations, which coreset seems to have missed.}
    \label{fig:figure4}
\end{figure*}


==> other_tex/prompt_complex.tex <==
\begin{listing}[!ht]
\begin{minted}[fontsize=\footnotesize, frame=single, breaklines]{python}
f'''
The following are {N} candidate instructions that describe a task, each indicated by a number identifier [].

[1]

### Instruction: {Example #1 Instruction}
### Input: {Example #1 Input}

...

### Instruction: {Example #N Instruction}
### Input: {Example #N Input}

Examine the provided list of {N} instructions, each uniquely identified by a number in brackets []. Your task is to select {num} instructions that will be annotated by human annotators for model fine-tuning. Look for instructions that are clear and relevant, exhibit a high level of complexity and detail, represent a diverse range of scenarios and contexts, offer significant instructional value and potential learning gain, and present unique challenges and specificity. These selected instructions should ideally be the most beneficial for model fine-tuning after being annotated by human annotators. Present your selections using the format []. e.g., [1,2] or [2,3].

The most impactful {num} instructions (only identifiers) are:
'''
\end{minted}
\caption{Prompt of \name{}}
\label{lst:prompt_ours}
\end{listing}

==> other_tex/prompt_simple.tex <==
\begin{listing}[!ht]
\begin{minted}[fontsize=\footnotesize, frame=single, breaklines]{python}
f'''
Below are N passages related to the question at the end. After reading the passages, provide two correct candidates for the answer to the question at the end. Each answer should be in the form: (a) xx, (b) yy, and should not exceed 3 words for each candidate.

Passage #1 Title: {Passage #1 Title}
Passage #1 Text: {Passage #1 Text}

...

Passage #N Title: {Passage #N Title}
Passage #N Text: {Passage #N Text}

Question: {Question}

Answer:
'''
\end{minted}
\caption{Prompt for answer candidates generation.}
\label{lst:answer_candidates_generation}
\end{listing}

==> tables/main_cot.tex <==
\begin{table*}[t]
\small
\vspace{-0.1in}
\begin{center}
\caption{Reasonings generated by ChatGPT via zero-shot chain-of-thought \citep{kojima2022large} for selecting the relevant instructions.}
\label{table:examples_cot}
\begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \toprule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{1)}: \newline Instruction [6] was chosen because it meets several of the criteria for model fine-tuning. \newline \newline First, it is clear and relevant, asking for specific information about the location, founder, and nature of the Lollapalooza music festival. This specificity allows for a focused annotation task.\newline \newline Second, it exhibits a high level of complexity and detail. The instruction requires understanding and extraction of multiple pieces of information from the input text, including the location, founder, and description of the festival.\newline \newline Third, it represents a diverse range of scenarios and contexts. The task involves extracting information about a music festival, which is a distinct topic from the other instructions in the list.\newline \newline Fourth, it offers significant instructional value and potential learning gain. Annotating this instruction would help train the model to accurately extract specific details about events and their background information.\newline \newline Finally, it presents unique challenges and specificity. The instruction requires the model to identify and extract specific information about the location, founder, and nature of the Lollapalooza festival, which may require understanding and disambiguation of certain terms and concepts.\newline \newline Overall, annotating this instruction would contribute to the model's ability to accurately extract specific details about events and their background information, making it a valuable choice for model fine-t} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{2)}: \newline Instruction [7] was chosen because it meets several criteria for model fine-tuning. \newline \newline First, it is clear and relevant, asking for a definition and explanation of a specific concept ("What is process mining?"). This clarity ensures that the annotators will have a clear understanding of what is being asked and can provide a precise response.\newline \newline Second, it exhibits a high level of complexity and detail. The instruction provides a detailed description of process mining, including its techniques, goals, and the types of questions it can answer. This complexity will challenge the annotators to provide a comprehensive and accurate response.\newline \newline Third, it represents a diverse range of scenarios and contexts. Process mining is a technique used in various fields, such as data science and process management, making it applicable to different industries and domains. Annotating this instruction will expose the model to a diverse set of knowledge and terminology.\newline \newline Fourth, it offers significant instructional value and potential learning gain. Process mining is a specialized topic that requires domain-specific knowledge. Annotating this instruction will help the model understand and generate accurate responses to similar questions in the future.\newline \newline Finally, it presents a unique challenge and specificity. Process mining is a niche topic that may not be well-known to the general public. Annotating this instruction will require the} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{3)}: \newline Instruction [12] was chosen because it meets several criteria for model fine-tuning. \newline \newline First, it is clear and relevant, asking for a specific piece of information - the top speed of a Kia Stinger. This clarity ensures that the annotators will have a clear understanding of what is being asked.\newline \newline Second, it exhibits a high level of complexity and detail. The instruction provides a paragraph of information about the Kia Stinger, including different acceleration times and top speeds for different models. Annotators will need to carefully read and analyze this information to determine the correct answer.\newline \newline Third, it represents a unique context and scenario. The instruction asks for the top speed of a specific car model, which requires annotators to have knowledge about cars and their specifications. This adds variety to the types of instructions being annotated.\newline \newline Fourth, it offers significant instructional value and potential learning gain. Annotators will need to research and understand the information provided about the Kia Stinger to accurately answer the question. This process of researching and learning about a specific topic can be valuable for model fine-tuning.\newline \newline Overall, instruction [12] presents a specific and detailed task that requires research and knowledge in a specific domain. It offers potential learning gain for annotators and contributes to the diversity of annotated instructions.} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
\end{center}
\end{table*}








==> tables/main_examples.tex <==
\begin{table*}[t]
\small
\vspace{-0.1in}
\begin{center}
\caption{Examples of generated sentences.}
\label{table:examples}
\begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \toprule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: Where was Sarah Schechter born?} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Input}: Schechter was born in Boston and grew up in Brookline, Massachusetts and New York City. Her father, Danny Schechter, a grandson of Russian-Jewish immigrant socialists, was a human rights activist, author, filmmaker and television producer.} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Ground Truth}: Sarah Schechter was born in Boston, Massachusetts.} \\
        \midrule
        \textbf{Random} & \textbf{Coreset} & \textbf{Ours} \\
        \textit{Sarah Schechter was born in Boston and grew up in Brookline, Massachusetts and New York City. Her father, Danny Schechter, a grandson of Russian-Jewish immigrant socialists, was a human rights activist, author, filmmaker and television producer.\newline\newline
\#\#\# Instruction:\newline
            What is the name of the first book in the Harry Potter series?\newline\newline
            \#\#\# Input:\newline
            Harry Potter and the Philosopher's Stone\newline\newline
            \#\#\# Response:\newline
             Harry Potter and the Philosopher's Stone\newline\newline
\#\#\# Instruction:\newline
            What is the name of the first book in the Harry Potter series?\newline\newline
            \#\#\#} & \textit{Sarah Schechter was born in Boston and grew up in Brookline, Massachusetts and New York City. Her father, Danny Schechter, a grandson of Russian-Jewish immigrant socialists, was a human rights activist, author, filmmaker and television producer.} &\textit{Sarah Schechter was born in Boston, Massachusetts.
} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
    \begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \toprule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: Write an email to the head of academic coaching at Services for Students with Disabilities sharing that I've applied to the coaching position. I have experience volunteering with children on the autism spectrum.} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Ground Truth}: \newline Hi, \newline
        
        I hope you are having a wonderful day. My name is \_, and I just applied for the Program Staff position at the Services for Students with Disabilities to empower students who have disabilities to reach their academic dreams. My background working in higher education and volunteering with kids on the Autism spectrum combine to bring an empathetic and impactful perspective.\newline

        Please let me know if there is anything else I can do at this time to be considered for this position. \newline

        With gratitude,\newline
        \_} \\
        \midrule
        \textbf{Random} & \textbf{Coreset} & \textbf{Ours} \\
        \textit{\textcolor{red}{Dear Head of Academic Coaching},\newline\newline
            I am writing to share that I have applied to the coaching position. I have experience volunteering with children on the autism spectrum.\newline\newline
            Thank you for your time.\newline\newline
            Sincerely,\newline\newline
            Katie} & \textit{I’m writing to share that I’ve applied to the coaching position. I have experience volunteering with children on the autism spectrum.} &\textit{\textcolor{red}{Dear Head of Academic Coaching}, \newline \newline I am writing to share that I have applied to the coaching position. I have experience volunteering with children on the autism spectrum. \textcolor{blue}{I am passionate about helping children with disabilities and I believe that I would be a great asset to your team. I am confident that I can make a positive impact on the lives of the students that I work with.}
} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
\begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \toprule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: Which is a species of fish? Red snapper or Red Sox} \\
        \midrule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Ground Truth}: Red snapper} \\
        \midrule
        \textbf{Random} & \textbf{Coreset} & \textbf{Ours} \\
        \textit{Red snapper\newline\newline
\#\#\# Instruction:\newline
            What is the name of the first person to win the Tour de France?\newline\newline
            \#\#\# Input:\newline\newline
            \#\#\# Response:\newline
            Maurice Garin\newline\newline
\#\#\# Instruction:\newline
            What is the name of the first person to win the Tour de France?\newline\newline
            \#\#\# Input:\newline\newline\newline
            \#\#\# Response:\newline\newline
            Maurice Garin} & \textit{Red snapper is a species of fish.} &\textit{Red snapper is a species of fish.\newline
Red Sox is a baseball team.
} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
\end{center}
\end{table*}








==> tables/main_instructions.tex <==
\begin{table*}[t]
\small
\vspace{-0.1in}
\begin{center}
\caption{Chosen Instructions by SelectLLM}
\label{table:chosen}
    \begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \toprule
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: Explain how new technologies, like LLMs and ChatGPT, may revolutionize Application Programming Interfaces (APIs) in the future. Provide an example of how these APIs might work.} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
    \begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: Let’s solve the following math problem. Each rabbit has 4 feets and each duck has 2 feets. If there are in total 25 heads and 88 feets, how many rabbits and how many ducks are there?} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
    \begin{adjustbox}{width=1.0\linewidth}
    \begin{tabularx}{\textwidth}{@{}X|X|X@{}}
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Instruction}: From the text below extract the types of species and the percentage of its habitat in the form {Species}:{Percentage} and place them as a bullet list} \\
        \multicolumn{3}{@{}p{\textwidth}@{}}{\textbf{Input}: \newline India is a megadiverse country, a term employed for 17 countries which display high biological diversity and contain many species exclusively indigenous, or endemic, to them. India is a habitat for 8.6\% of all mammal species, 13.7\% of bird species, 7.9\% of reptile species, 6\% of amphibian species, 12.2\% of fish species, and 6.0\% of all flowering plant species. Fully a third of Indian plant species are endemic. India also contains four of the world's 34 biodiversity hotspots, or regions that display significant habitat loss in the presence of high endemism.} \\
        \bottomrule
    \end{tabularx}
    \end{adjustbox}
\end{center}
\end{table*}







